An Overview of Recent Work in Media Forensics: Methods and Threats

In this paper, we review recent work in media forensics for digital images, video, audio (specifically speech), and documents. For each data modality, we discuss synthesis and manipulation techniques that can be used to create and modify digital media. We then review technological advancements for detecting and quantifying such manipulations. Finally, we consider open issues and suggest directions for future research.

==> part-7-fusion.tex <==
%\section{Fusion}\label{part-7-fusion}

% Multimedia assets have more than one media present \eg a video has image sequences and audio sequences, and news articles have text along with images.
% Recent developments in deep learning have made it easy to individually generate deepfake audio, image, and video.
% It is still challenging to generate deepfake video or fake articles that are consistent in terms of high-level semantic features.
% This can be exploited to detect deepfakes.
% For example, in \cite{hosler2021do}, the authors detected deepfake videos of humans by analyzing both audio and image sequences individually by looking for emotional inconsistencies across them. 


% Audio and image sequences were divided into temporal segments.
% For each audio segment using speech features, an LSTM predicted valence (\ie subject’s emotional affect - positive to negative) and arousal (\ie the magnitude of that emotion).
% For each image sequence segment, a similar LSTM using facial features predicted valence and arousal.
% Once the arousal and valence over time in the visual and audio domains are available, the Lin’s Concordance Correlation Coefficient \cite{hosler2021do} estimated the correlation across the domain for same features.
% This detects deepfake videos by capturing the inconsistency of arousal and valence across domains. 
